Divergence-Preserving Branching Bisimilarity

This note considers the notion of divergence-preserving branching bisimilarity. It briefly surveys results pertaining to the notion that have been obtained in the past one-and-a-half decade, discusses its role in the study of expressiveness of process calculi, and concludes with some suggestions for future work.

==> eptcsdata.tex <==
\providecommand{\firstpage}{3}
\providecommand{\publicationstatus}{O. Dardha and J. Rot (Eds.): Combined Workshop on Expressiveness in \\ Concurrency and Structural Operational Semantics (EXPRESS/SOS 2020).\\
EPTCS 322, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.322.2}{10.4204/EPTCS.322.2}}

